Recurrent Deep Divergence-based Clustering for simultaneous feature learning and clustering of variable length time series

The task of clustering unlabeled time series and sequences entails a particular set of challenges, namely to adequately model temporal relations and variable sequence lengths. If these challenges are not properly handled, the resulting clusters might be of suboptimal quality. As a key solution, we present a joint clustering and feature learning framework for time series based on deep learning. For a given set of time series, we train a recurrent network to represent, or embed, each time series in a vector space such that a divergence-based clustering loss function can discover the underlying cluster structure in an end-to-end manner. Unlike previous approaches, our model inherently handles multivariate time series of variable lengths and does not require specification of a distance-measure in the input space. On a diverse set of benchmark datasets we illustrate that our proposed Recurrent Deep Divergence-based Clustering approach outperforms, or performs comparable to, previous approaches.

==> commands.tex <==
%!TEX root = main.tex
\makeatletter
\def\lrp#1{\left(#1\right)}
% Automatic left-right parenthesis for if next character is
% an opening bracket. Example:
% \autolrp\sin % has the following effect:
% \sin{sum_{i=1}^{\infty}} <-> \sin\left(sum_{i=1}^{\infty}\right)
% whilst \sin and \sin(\omega) won't complain and won't do \left and \right.
\def\@autolrp{\@ifnextchar\bgroup\lrp\relax}
\def\autolrp#1{\g@addto@macro#1\@autolrp}

\def\@autopow{\@ifnextchar\bgroup^\relax}
\def\autopow#1{\g@addto@macro#1\@autopow}


\autolrp\sin
\autolrp\cos
\def\e{\@ifnextchar^{\mathrm{e}}{\mathrm{exp}\!\@autolrp}}

\def\opFont#1{{\operator@font #1}}
\makeatother

\let\vec\undefined
\def\vec#1{\mathbf{#1}}
\let\mat\vec
\let\v\vec



% \vec for Greek-letter
\def\gvec#1{\boldsymbol{#1}}

\let\cl\mathcal
\def\real{\mathbb{R}}

\DeclareMathOperator{\triu}{triu}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\E}{\mathbb{E}}

\def\lrp#1{\left(#1\right)}
\def\sums#1#2{\sum\limits_{#1}^{#2}}
\def\T{^T}

\newcommand{\numberthis}{\addtocounter{equation}{1}\tag{\theequation}}%Number equation%
\makeatletter
\if@todonotes@disabled%
  \newcommand\todomark[2][]{\relax}\else%
  \newcommand\todomark[2][orange]{{\color{#1}\large(}#2{\color{#1}\large)}}%
\fi

\newcommand{\resizeinput}[2][\textwidth]{\resizebox{#1}{!}{\input{#2}}}

\newcommand{\thickhline}{%
    \noalign {\ifnum 0=`}\fi \hrule height 2pt
    \futurelet \reserved@a \@xhline
}
\newcommand\ifspacemagic{\ifcsname spacemagic\endcsname\@firstoftwo\else\@gobble\fi}


==> fig/ddc.tex <==
\begin{tikzpicture}[node distance=1cm]
  \tikzstyle{nn} = [rectangle, rounded corners, minimum width=3cm, minimum height=3cm,text centered, draw=black, fill=green!20]
  \tikzstyle{fc} = [rectangle, rounded corners, minimum width=1cm, minimum height=3cm,text centered, draw=black, fill=red!20]
  \tikzstyle{K} = [rectangle, rounded corners, minimum width=1cm, minimum height=1cm,text centered, draw=black]
  \tikzstyle{input} = [rectangle, minimum width=3cm, minimum height=0.7cm,text centered, draw=black]
  \tikzstyle{arrow} = [thick,->,>=stealth]

  \node (fm) [nn] {RNN};
  \node (in) [input, below of=fm, yshift=-1.5cm] {Input};%{\( \vec x_1, \dots, \vec x_T \)};
  \node (bn) [K, right of=fm, xshift=2cm] {BN};
  \node (fc1) [fc, right of=bn, xshift=1cm] {FC};
  \node (fc2) [fc, right of=fc1, xshift=1.5cm] {Out};
  \node (Kh) [K, above of=fc2, yshift=1.5cm] {\( \mat K_h \)};
  \node (Loss) [K, right of=fc2, xshift=1.5cm] {\( \mathcal{L} \)};

  \draw [arrow] (in) -- (fm);
  \draw [arrow] (fm) -- (bn);
  \draw [arrow] (bn) -- (fc1) node [midway,below] {\( \vec y \)};
  \draw [arrow] (fc1) -- (fc2) node [midway,below] {\( \vec h \)};
  \draw [arrow] (fc1) -- (Kh) node [midway,above,xshift=-0.2cm] {\( \vec h \)};
  \draw [arrow] (fc2) -- (Loss) node [midway,below] {\( \vec \alpha \)};
  \draw [arrow] (Kh) -- (Loss); %node [midway,above,xshift=0.2cm] {\( \mat K_h \)};
\end{tikzpicture}


==> fig/rddc/simplexPoints.tex <==
%!TEX root = main.tex% This file is generated by pointgen.py\node[point] at (33.0pt, -0.6666301580481071pt) {};
\node[point] at (25.0pt, -3.404827860134042pt) {};
\node[point] at (30.37463977675479pt, -0.03794822364003662pt) {};
\node[point] at (32.221934906342284pt, -4.107416553865756pt) {};
\node[point] at (29.07587452261009pt, -3.722579149857764pt) {};
\node[point] at (29.1305556291578pt, 2.4843835384255817pt) {};
\node[point] at (28.14018282627439pt, 2.360180136713102pt) {};
\node[point] at (28.774818671692053pt, 1.4399187805304479pt) {};\node[point] at (1.7349941131833828pt, 29.739086444256706pt) {};
\node[point] at (-0.8033960620362428pt, 26.821813392369144pt) {};
\node[point] at (0.8538480707692049pt, 29.129161356521017pt) {};
\node[point] at (0.3593450552260344pt, 33.0pt) {};
\node[point] at (1.9977277788234908pt, 29.657275713352142pt) {};
\node[point] at (-0.18871636036075207pt, 26.490132924026657pt) {};
\node[point] at (1.2633402749953413pt, 27.734034382194235pt) {};
\node[point] at (0.8057536344039301pt, 25.0pt) {};

==> fig/rddc/tikzhelpers.tex <==
%!TEX root = main.tex
\makeatletter
\usepackage{tikz}
\usepackage{listofitems}
\usepackage{pgfplots}
\usepackage{pgf,tikz}
\usepackage{mathrsfs}
% \pgfplotsset{compat=1.15}
\let\dlog\@latex@warning
\newcommand\calcdef[2]{
	\pgfmathparse{#2}\xdef#1{\pgfmathresult}
}
\def\pgfexpkeys#1{
\edef\expanded@keys{{#1}}
\expandafter\pgfkeys\expanded@keys
}
% /NN/neurons/.meta tikz style={tikz/path}
% Now, when /NN/neurons={grey} it also sets /tiks/path/.style={grey}.
\pgfkeys{%
	/handlers/.meta tikz style/.code={%
			\pgfkeys{\pgfkeyscurrentpath/.code={\pgfkeysalso{/tikz/#1/.style={##1}}}}
  },
  % /NN/neurons/.meta append tikz style={tikz/path}{base style}
  % Now, when /NN/neurons={grey} it also sets /tiks/path/.append style={grey}.
  /handlers/.meta append tikz style/.code 2 args={%
		  \pgfkeys{\pgfkeyscurrentpath/.code={\pgfkeys{/tikz/#1/.style={#2}}\pgfkeysalso{/tikz/#1/.append style={##1}}}}
  },
  /handlers/.settable style/.code={\pgfkeys{\pgfkeyscurrentpath/.code=\pgfkeysalso{##1}}}
}
\pgfdeclarelayer{foreground}
\pgfdeclarelayer{background}
\pgfdeclarelayer{wallpaper}
\pgfdeclarelayer{wall}
\pgfsetlayers{wall,wallpaper,background,main,foreground}   %% some additional layers for demo
\usetikzlibrary{fit,calc}
\tikzset{
	fitting node/.style={
			inner sep=0pt,
			fill=none,
			draw=none,
			% reset transform,
			fit={(\pgf@pathminx,\pgf@pathminy) (\pgf@pathmaxx,\pgf@pathmaxy)}
		},
	reset transform/.code={\pgftransformreset},
	set dim/.style={insert path={%
					coordinate [pos=0] (tmpa)
					coordinate [pos=1] (tmpb)
					\pgfextra{%
						\pgfextractx{\pgf@x}{\pgfpointanchor{tmpa}{center}}
						\pgfextracty{\pgf@y}{\pgfpointanchor{tmpa}{center}}
						\pgf@xa\pgf@x %
						\pgf@ya\pgf@y %
						\pgfextractx{\pgf@x}{\pgfpointanchor{tmpb}{center}}
						\pgfextracty{\pgf@y}{\pgfpointanchor{tmpb}{center}}
						\pgf@xb\pgf@x %
						\pgf@yb\pgf@y %
						\advance\pgf@xb by -\pgf@xa
						\advance\pgf@yb by -\pgf@ya
					}%
				}, minimum width=\pgf@xb,minimum height=\pgf@yb
		}%
}%
\tikzset{
    partial ellipse/.style args={#1:#2:#3}{
        insert path={+ (#1:#3) arc (#1:#2:#3)}
    }
}
\usetikzlibrary{arrows}
% \pagestyle{empty}

\newdimen\tmp@tikz@x
\newdimen\tmp@tikz@y
% Extract x and y components from coordinate
% \extractCoords[anchor]{COORDINATE}{outputPrefix}
% Defines \outputPrefix@x, \outputPrefix@y and \outputPrefix@xy -> x,y
\newcommand\extractCoords[3][center]{%
	\pgfextractx{\tmp@tikz@x}{\pgfpointanchor{#2}{#1}}%
	\pgfextracty{\tmp@tikz@y}{\pgfpointanchor{#2}{#1}}%
	\expandafter\xdef\csname #3@xy\endcsname{\the\dimexpr\tmp@tikz@x,\the\dimexpr\tmp@tikz@y}%
	\expandafter\xdef\csname #3@x\endcsname{\the\dimexpr\tmp@tikz@x}%
	\expandafter\xdef\csname #3@y\endcsname{\the\dimexpr\tmp@tikz@y}%
}
\def\excoord(#1){%
\edef\coordname{(#1)}%
\expandafter\coordinate\coordname%
}
\makeatother


==> fig/rddc/timeseries.tex <==
%!TEX root = main.tex
%% Comma separated list of the signals
\edef\colors{red,green,blue,black,magenta,cyan}
%% The z-values contains the depth coordinate of the signal
\edef\ZValues{0.5,1.5,2.5,3.5,4.5,5.5}
%% Amplitude of all signals
\edef\amplitude{0.4}
\edef\xOffset{-0.25}
%% Read the lists for index handling
\readlist*\clrlist\colors
\readlist*\zlist\ZValues
\begin{scope}[
    x={(0:1)},
    y={(90:1)},
    z={(0,0)},
    rotate around z=0,
    rotate around x=20,
    rotate around y=-40
  ]
  %% Axes
  \coordinate(origin) at (0,0,0);
  \coordinate(times-anchor) at (3.25,0,0);
  \draw[blue!90] (origin) --++ (6.5,0,0) node[right]{};
  % \draw[->, blue!90] (origin) --++ (0,1,0) node[right]{y};
  \draw[blue!90] (origin) --++ (0,0,6.5) node[right]{};
  %% Foreach "signal"
  \foreach \idx in {1,...,\zlistlen}{
    %% Get z-value and color
    \edef\z{\zlist[\idx]}
    \edef\clr{\clrlist[\idx]}
    % Draw signal with (50%) color
    \begin{pgfonlayer}{main}
    \draw[\clr!80, thick](0,0,\z)%
        \foreach \x in {0.00,0.01,...,6.28}{
            --({\x},{\amplitude*(sin((sqrt(\z)*(\x+\xOffset)*170))+1)},{\z})
            % --({\x},{\amplitude*(sin((3.75*sqrt(\z)*\x-1.57)*180/3.14)+1)},{\z})
          };
    \end{pgfonlayer}
    %% Draw grey line below signal
    \begin{pgfonlayer}{wall}
      \draw[gray](0,0,\z) -- ++(6.28,0,0);
    \end{pgfonlayer}
  };
\end{scope}

